Beyond Observed Auxiliary Relations: Environment-Conditioned Modeling for Multi-Behavior Recommendation

Multi-behavior recommendation (MBR) leverages auxiliary behavioral signals, such as clicks and add-to-cart, to enhance target behavior prediction like purchases. While recent graph neural network-based approaches have achieved strong performance by systematically propagating auxiliary behavior signals, they still suffer from two fundamental challenges inherent to auxiliary behaviors: (1) missing auxiliary signals, which hinder generalization to items without auxiliary observations, and (2) unreliable auxiliary signals, which amplify noise misaligned with the target behavior. To address these challenges in a unified manner, we propose BOAR, an environment-conditioned MBR framework that addresses missing and unreliable auxiliary signals through two complementary modules conditioned on auxiliary observability. Extensive experiments demonstrate that BOAR consistently outperforms state-of-the-art baselines, achieving up to 7.82% gains in HR@10 overall and up to 44.2% gains for target items without auxiliary observations, highlighting its ability to capture hidden preferences beyond observed auxiliary relations. Our code is available at: https://github.com/LSH0411/BOAR.

==> sections/031Preliminaries_v1.tex <==
\subsection{Problem Formulation}
Let $\mathcal{U}$ and $\mathcal{I}$ denote the sets of users and items. % ($M=|\mathcal{U}|$, $N=|\mathcal{I}|$).
We consider a set of behaviors $\mathcal{B}=\{b_1,\ldots,b_{|\mathcal{B}|}\}$ (e.g., click, cart, ... , buy), where $b_{\mathrm{tar}}=b_{|\mathcal{B}|}$ is the target behavior and $\mathcal{B}\setminus\{b_{\mathrm{tar}}\}$ are auxiliary behaviors.
For each behavior $b\in\mathcal{B}$, we define a bipartite graph $\mathcal{G}_b=(\mathcal{U}\cup\mathcal{I},\mathcal{E}_b)$, where $\mathcal{E}_b\subseteq\mathcal{U}\times\mathcal{I}$ denotes the observed interactions.
% $\mathbf{A}_{b}$ denotes the corresponding adjacency matrix.
For each pair $(u,i)$, we define a binary random variable $R_{ui}\in\{0,1\}$ indicating whether user $u$ engages in the target behavior on item~$i$.
Our goal is to learn a function $f(u,i)$ that estimates the probability that a user $u$ exhibits the target behavior with item $i$:
\begin{equation}
f(u,i)\ \approx\ \mathbb{E}\!\left[R_{ui}\mid u,i\right]\ =\ P(R_{ui}=1\mid u,i).
\end{equation}
We focus on addressing the aforementioned challenges, \textbf{C1}: missing auxiliary signals and \textbf{C2}: unreliable auxiliary signals, arising from the nature of auxiliary behaviors.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/imbalance.pdf}
    \caption{Data imbalance between auxiliary and target interactions on the Tmall dataset (left) and its impact on the performance gap between auxiliary-observed and hidden target items (right).}
    \label{fig:figure0}
    \vspace{-0.3cm}
\end{figure}

\subsection{Environment-Conditioned Modeling}
\label{subsec:env_modeling}
In terms of target behavior prediction, target-positive items can be categorized into
(i) \textit{hidden} target items, which have no auxiliary interactions, and
(ii) \textit{observed} target items, which are associated with auxiliary behaviors (Figure~\ref{fig:figure1}).
As auxiliary observability substantially affects target behavior prediction, holistic modeling of user--item interactions may obscure such differences and lead to suboptimal results.


\noindent
\textbf{Motivation for Environment Modeling.}
As shown in Figure~\ref{fig:figure0} (left), auxiliary interactions substantially outnumber target interactions, causing GNN-based models to develop biases toward auxiliary-observed items.
This imbalance directly leads to the performance gap shown in Figure~\ref{fig:figure0} (right): even state-of-the-art methods show a significant drop on hidden target items.
This gap suggests that holistic modeling without auxiliary-observability awareness often struggles to predict hidden preference items, motivating a modeling approach that accounts for auxiliary observability.

\noindent
\textbf{Environment Modeling by Auxiliary Observability.}
To explicitly account for this heterogeneity, we distinguish user–item pairs according to the presence of auxiliary interactions.
Let $\mathcal{E}_{\text{aux}}=\bigcup_{b\in \mathcal{B}\setminus\{b_{\mathrm{tar}}\}}\mathcal{E}_b$ denote the set of all observed auxiliary interactions.
We define the environment indicator as follows:
\begin{equation}
\label{env_indicator}
E_{ui}=
\begin{cases}
0, & (u,i)\notin \mathcal{E}_{\text{aux}} \quad \text{(auxiliary-unobserved)},\\
1, & (u,i)\in \mathcal{E}_{\text{aux}} \quad \text{(auxiliary-observed)}.
\end{cases}
\end{equation}
% This definition is fully observable from interaction logs and partitions the pair space into two environments with distinct challenges.
While C1 and C2 are not independent challenges, their adverse effects manifest with different prominence across the~environments.
\begin{itemize}[leftmargin=*, labelsep=0.5em, topsep=3pt, itemsep=3pt]
    \item \textbf{Environment 0 ($E_{ui}=0$)} requires identifying hidden target items among a vast number of unobserved items.
    This is particularly difficult because auxiliary interactions are limited and heavily biased toward a small set of items, hindering generalization to broad unobserved items.
    
    \item \textbf{Environment 1 ($E_{ui}=1$)} requires identifying which observed items will lead to the target behavior.
    Because auxiliary behaviors may reflect incidental or non-purchase intent, propagating such signals can amplify irrelevant information and cause models to misinterpret auxiliary signals as purchase intent.
\end{itemize}
% This partitioning highlights that target behavior prediction exhibits different failure patterns across environments.
% This partitioning highlights that prediction exhibits different failure patterns, with the effects of C1 and C2 being more prominent in each environment, respectively.
This distinction highlights different failure patterns, where the effects of C1 and C2 tend to be more prominent depending on the presence of auxiliary interactions, respectively.
This asymmetry suggests that auxiliary observability serves as the partition boundary for the two challenges, as finer-grained splits (e.g., by behavior type) would not alter the fundamental challenge type in each region; the diversity and varying importance of auxiliary behaviors are explicitly addressed within each module.

\noindent
\noindent
\textbf{Environment-Conditioned Modeling.}
This formulation naturally motivates a modular perspective, in which target preference estimation is conditioned on the environment.
By the law of total expectation, the target preference can be decomposed as:
\begin{equation}
\label{eq:total_expectation}
\mathbb{E}[R_{ui}\mid u,i]
= \sum_{e\in\{0,1\}} P(E_{ui}{=}e\mid u,i)\ \mathbb{E}[R_{ui}\mid u,i,E_{ui}{=}e].
\end{equation}
Accordingly, we consider modeling the conditional expectations with two environment-conditioned sub-modules:
\begin{equation}
\begin{aligned}
f_0(u,i) &\approx \mathbb{E}[R_{ui}\mid u,i,E_{ui}{=}0],\\
f_1(u,i) &\approx \mathbb{E}[R_{ui}\mid u,i,E_{ui}{=}1].
\end{aligned}
\end{equation}
The final prediction is obtained by aggregating the conditional predictions as $f(u,i)
= \sum_{e\in\{0,1\}} P(E_{ui}=e \mid u,i)\, f_e(u,i)$.
This modular formulation establishes a unified framework for capturing distinct interaction patterns.
The concrete instantiation is introduced in the subsequent section.






% Importantly, this substantial gap reveals not merely a quantitative difference but a structural one: accurate prediction in the auxiliary-unobserved environment requires densifying the sparse target graph by recovering hidden preferences, whereas the auxiliary-observed environment demands pruning auxiliary relations that are misaligned with the target behavior.



==> sections/041Method_backup.tex <==
% ===============================
% Proposed Method 
% ===============================
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/method.pdf}
    % \includegraphics[width=\textwidth, trim={0 0 0 0}, clip]{figs/overview_method.pdf}
    \caption{Overview of the proposed method.}
    \label{fig:overview_method}
\end{figure*}

We introduce \textbf{\textsc{BOAR}} (Beyond Observed Auxiliary Relations), a MBR framework derived from the environment-aware modeling.
An overview of the overall framework is provided in Figure~\ref{fig:overview_method}.
\textsc{BOAR} comprises two specialized modules, each optimized for its corresponding environment.

\begin{itemize}[leftmargin=*, labelsep=0.5em, topsep=3pt, itemsep=3pt]
    \item \textbf{Environment 0 (auxiliary-unobserved).}
    The \textit{Debiased Densification Module} ($f_0$) addresses the incompleteness and bias of auxiliary behaviors by recovering hidden preferences.

    \item \textbf{Environment 1 (auxiliary-observed).}
    The \textit{Selective Pruning Module} ($f_1$) addresses the discrepancy between auxiliary and target behaviors by suppressing noisy auxiliary signals via target-gated pruning.
\end{itemize}

\noindent
The two modules are optimized with environment-specific objectives and parameters.


\subsubsection{\textbf{Base Encoding.}}
\label{sec:unobserved_base}
We first compute base user/item representations that serve as the starting point for subsequent environment-specific modeling.
We adopt \emph{LightGCN}~\cite{LightGCN} as the graph encoder and denote it by $\mathrm{LGCN}(\cdot)$.
\begin{equation}
\mathbf{E}^{\mathrm{glo}} = \mathrm{LGCN}\!\left(\mathbf{E}^{\mathrm{init}}, \mathcal{G}_{\mathrm{glo}}\right), \qquad
\mathbf{E}^{\mathrm{tar}} = \mathrm{LGCN}\!\left(\mathbf{E}^{\mathrm{init}}, \mathcal{G}_{\mathrm{tar}}\right).
\end{equation}

\noindent
Where, $\mathbf{E}^{\mathrm{glo}}$ denotes the \emph{global} user--item embedding matrix encoded on the global graph $\mathcal{G}_{\mathrm{glo}}$, and $\mathbf{E}^{\mathrm{tar}}$ denotes the embedding matrix encoded on the target graph $\mathcal{G}_{\mathrm{tar}}$.
The global graph $\mathcal{G}_{\mathrm{glo}}$ is constructed from the union of all behavior interaction sets, i.e., $\mathcal{E}_{\mathrm{glo}}=\bigcup_{b\in\mathcal{B}} \mathcal{E}_b$.



% \subsection{Base Graph Encoding}
% Let $\mathcal{G}=(\mathcal{U} \cup \mathcal{V}, \mathcal{E})$ denote the interaction graph, where $\mathcal{U}$ and $\mathcal{V}$ represent the sets of users and items, respectively.
% We adopt LightGCN~\cite{LightGCN} as the backbone encoder to capture high-order connectivities. 
% The initial embeddings are parameterized as $\mathbf{E}^{(0)} \in \mathbb{R}^{(|\mathcal{U}|+|\mathcal{V}|) \times d}$.
% The graph propagation at the $l$-th layer is defined as:
% \begin{equation}
%     \mathbf{e}_u^{(l+1)} = \sum_{v \in \mathcal{N}_u} \frac{1}{\sqrt{d_u d_v}} \mathbf{e}_v^{(l)}, \quad
%     \mathbf{e}_v^{(l+1)} = \sum_{u \in \mathcal{N}_v} \frac{1}{\sqrt{d_u d_v}} \mathbf{e}_u^{(l)},
% \end{equation}
% where $d_u$ and $d_v$ denote the degrees of user $u$ and item $v$.
% The final representations $\mathbf{e}_u, \mathbf{e}_v$ are obtained by mean-pooling the embeddings from all $L$ layers. These embeddings serve as the input for the subsequent environment-specific modeling.

\label{sec:unobserved}

\subsection{Auxiliary-Unobserved Environment Modeling}
In the auxiliary-unobserved environment ($E_{ui} = 0$), user-item pairs lack explicit auxiliary signals, making preference inference challenging due to incomplete observations.
To address this, we propose a debiased densification strategy that consists of three key components: (1) \textit{auxiliary observation-invariant learning} to mitigate observation bias by learning representations that are invariant to auxiliary behavior patterns, (2) \textit{target hidden preference miner} to efficiently discover high-confidence hidden preferences through locality-sensitive hashing and learnable candidate selection, and (3) \textit{hidden preference robust transfer} to safely inject the mined knowledge into the representation space via self-supervised contrastive learning, avoiding false supervision from potentially noisy candidates.

\subsubsection{\textbf{Auxiliary Observation-Invariant Learning.}}

The global embeddings should encode representations that generalize to the auxiliary-unobserved environment, where no auxiliary signals are available.
A key challenge arises when auxiliary-observed and unobserved pairs exhibit distinguishable representation patterns.
In such cases, the model may exploit this shortcut by relying on auxiliary-observability cues (e.g., popular items) rather than capturing true user-specific purchase intent, degrading its ability to recommend hidden target-positive items that lack auxiliary interactions.


To address this, we enforce \emph{auxiliary observation-invariant} representations by making auxiliary-observed and auxiliary-unobserved pairs indistinguishable in the global embedding space.
This is achieved through adversarial training with a gradient reversal layer, which prevents auxiliary-observability patterns from being encoded while preserving genuine preference signals.


Specifically, we construct a domain-labeled set $\mathcal{S}_{\mathrm{dom}}$ consisting of two types of pairs: (1) auxiliary interactions that do not overlap with target behavior $\mathcal{S}_{\mathrm{aux}} = \{(u,i,b) \mid (u,i) \in \mathcal{E}_b \setminus \mathcal{E}_{\mathrm{tar}}, b \in \mathcal{B} \setminus \{b_{\mathrm{tar}}\}\}$, and (2) auxiliary-unobserved pairs $\mathcal{S}_{\mathrm{unobs}} = \{(u,i,\mathrm{unobs}) \mid (u,i) \notin \mathcal{E}_{\mathrm{glo}}\}$. By excluding target-overlapping interactions, we preserve target preference signals while removing auxiliary-specific observability cues. Each sample is assigned a domain label $c \in (\mathcal{B} \setminus \{b_{\mathrm{tar}}\}) \cup \{\mathrm{unobs}\}$, distinguishing each auxiliary behavior type (e.g., click, cart) from the unobserved status.

Given global embeddings $\mathbf{e}^{\mathrm{glo}}_u$ and $\mathbf{e}^{\mathrm{glo}}_i$, we concatenate them to form pair representation $\mathbf{z}_{ui} = [\mathbf{e}^{\mathrm{glo}}_u \| \mathbf{e}^{\mathrm{glo}}_i]$. A domain classifier $f_{\phi}$ (implemented as an MLP) is trained to predict the domain label, while the GRL adversarially updates the encoder to maximize classification error:
\begin{equation}
\mathbf{p}_{ui} = \mathrm{Softmax}(f_{\phi}(\mathrm{GRL}(\mathbf{z}_{ui}))), \quad
\mathcal{L}_{\mathrm{dom}} = \mathbb{E}_{(u,i,c) \sim \mathcal{S}_{\mathrm{dom}}}[-\log \mathbf{p}_{ui}[c]].
\end{equation}
This adversarial objective encourages the global embedding to learn representations where auxiliary-observed and unobserved pairs become indistinguishable, thereby mitigating auxiliary observation bias and enabling robust preference estimation in the unobserved environment.

\subsubsection{\textbf{Target Hidden Preference Miner.}}

In the auxiliary-unobserved environment, we infer potential target preferences for items with which users have no observed interactions.
Existing GR methods compute pairwise similarity across all user-item pairs to mine candidate edges~\cite{SHaRe,starline}, incurring prohibitive computational cost.
To address this, we propose a three-stage efficient mining strategy: (i) locality-sensitive hashing (LSH) for fast candidate retrieval, (ii) learnable edge selection to refine candidates, and (iii) weighted graph augmentation for target encoding.

\vspace{0.25em}
\noindent\textbf{Angular-LSH hashing.}
To efficiently retrieve candidate items without exhaustive similarity computation, we adopt angular LSH ~\cite{lsh,reformer}.
We draw a random projection matrix $\mathbf{R} \in \mathbb{R}^{d \times d'}$ with i.i.d. entries $R_{pq} \sim \mathcal{N}(0,1)$, and compute a signed concatenated projection for each node $x \in \mathcal{U} \cup \mathcal{I}$ as $\mathbf{s}_x = \left[ \left( \frac{\mathbf{e}^{\mathrm{glo}}_x}{\| \mathbf{e}^{\mathrm{glo}}_x \|} \right)^\top \mathbf{R} \bigg\Vert \left( \frac{\mathbf{e}^{\mathrm{glo}}_x}{\| \mathbf{e}^{\mathrm{glo}}_x \|} \right)^\top (-\mathbf{R}) \right] \in \mathbb{R}^{2d'}$.
The hash bucket is assigned by $h(x) = \arg\max_k (\mathbf{s}_x)_k$, grouping nodes with similar angular directions.
For each user $u$, we collect items in the same bucket $\mathcal{N}_{\mathrm{LSH}}(u) = \{i \in \mathcal{I} \mid h(i) = h(u)\}$, exclude already observed neighbors $\mathcal{N}_{\mathrm{glo}}(u) = \{i \mid (u,i) \in \mathcal{E}_{\mathrm{glo}}\}$, and retrieve top-$K$ items by cosine similarity to form the candidate set $\mathcal{E}_{\mathrm{cand}}(u)$. We aggregate candidates across all users as $\mathcal{E}_{\mathrm{cand}} = \bigcup_{u \in \mathcal{U}} \{(u,i) \mid i \in \mathcal{E}_{\mathrm{cand}}(u)\}$.

\vspace{0.25em}
\noindent\textbf{Learnable candidate edge selection.}
Since LSH-based retrieval is an approximate candidate retrieval step, the retrieved bucket-level candidates may include noisy or weakly related pairs; thus, we further refine them through learnable filtering.
For each candidate pair $(u,i) \in \mathcal{E}_{\mathrm{cand}}$, we predict a binary add/drop decision using an MLP $f_{\mathrm{add}}$ that takes the concatenated pair embedding as input. We apply Gumbel-Softmax reparameterization~\cite{gumbel} to obtain a differentiable discrete selection:
\begin{equation}
\begin{split}
\mathbf{z}^{\mathrm{add}}_{ui} &= f_{\mathrm{add}}([\mathbf{e}^{\mathrm{glo}}_u \parallel \mathbf{e}^{\mathrm{glo}}_i]), \\
\mathbf{y}^{\mathrm{add}}_{ui} &= \mathrm{GumbelSoftmax}(\mathbf{z}^{\mathrm{add}}_{ui}; \tau), \\
m^{\mathrm{add}}_{ui} &= \mathbf{y}^{\mathrm{add}}_{ui}[0] \in \{0,1\}.
\end{split}
\end{equation}
This learnable selection mitigates the uncertainty inherent in hashing by adaptively filtering candidates based on learned preference patterns.

\vspace{0.25em}
\noindent\textbf{Edge weighting and target-graph augmentation.}
For selected candidate edges, we assign confidence weights that capture both angular alignment and magnitude consistency. Following~\cite{chen2024dualdomaincollaborativedenoisingsocial}, we compute a fused similarity combining normalized cosine similarity and Gaussian kernel on Euclidean distance:
\begin{equation}
w_{ui} = \frac{1}{2}\Big(1 + \cos(\mathbf{e}^{\mathrm{glo}}_u, \mathbf{e}^{\mathrm{glo}}_i)\Big) \cdot \exp\!\left(-\frac{1}{2\sigma^2} \|\mathbf{e}^{\mathrm{glo}}_u - \mathbf{e}^{\mathrm{glo}}_i\|_2^2\right).
\end{equation}
We then construct the final edge weight by preserving original target edges with weight 1 and assigning $m^{\mathrm{add}}_{ui} \cdot w_{ui}$ to selected candidates, keeping unselected pairs at weight 0. The augmented target edge set is formed as $\tilde{\mathcal{E}}_{\mathrm{tar}} = \mathcal{E}_{\mathrm{tar}} \cup \{(u,i) \in \mathcal{E}_{\mathrm{cand}} \mid m^{\mathrm{add}}_{ui} = 1\}$, and we encode the refined target representation via $\tilde{\mathbf{E}}_{\mathrm{tar}}= \mathrm{LGCN}(\mathbf{E}^{\mathrm{glo}}, \tilde{\mathcal{E}}_{\mathrm{tar}})$.

\subsubsection{\textbf{Hidden Preference Robust Transfer SSL}}
The mined candidate edges provide a \emph{hypothesis} about users' hidden target preferences in the auxiliary-unobserved environment.
However, these edges are inevitably noisy: a fraction of selected pairs may be \emph{spurious} due to approximation errors in mining.
Directly treating such estimated edges as positives in a ranking objective can induce \emph{false supervision}, leading to biased gradients and potentially causing \emph{ranking collapse} by over-amplifying incorrect user--item affinities.
To inject the mined knowledge in a safer and more robust manner, we transfer it via \emph{self-supervised contrastive learning} rather than direct pairwise ranking supervision.
Concretely, we apply an InfoNCE loss to align the target embeddings obtained from the original target graph and the augmented target graph.

Formally, the user-side transfer loss is defined as
\begin{equation}
\mathcal{L}^{user}_{ssl}
= - \sum_{u\in\mathcal{U}}
\log
\frac{\exp\big(\mathrm{sim}(\mathbf{e}^{\mathrm{tar}}_{u},\tilde{\mathbf{e}}^{\mathrm{tar}}_{u})/\tau\big)}
{\sum_{u'\in\mathcal{U}} \exp\big(\mathrm{sim}(\mathbf{e}^{\mathrm{tar}}_{u},\tilde{\mathbf{e}}^{\mathrm{tar}}_{u'})/\tau\big)}.
\end{equation}
We compute the item-side loss $\mathcal{L}^{item}_{ssl}$ analogously by replacing users with items, and define the overall robust transfer objective as
\begin{equation}
\mathcal{L}^{(unob)}_{ssl}=\mathcal{L}^{user}_{ssl}+\mathcal{L}^{item}_{ssl},
\end{equation}
where $\mathrm{sim}(\cdot,\cdot)$ denotes similarity function (e.g., cosine similarity) and $\tau$ is the temperature hyperparameter.

\label{sec:observed}
\subsection{Auxiliary-Observed Environment Modeling}
In the auxiliary-observed environment ($E_{ui} = 1$), user-item pairs have rich auxiliary signals but suffer from noise and semantic misalignment with the target behavior.
To exploit these signals while suppressing irrelevant information, we propose a selective pruning strategy with two main components: (1) \textit{target-gated pruning graph encoder} that performs layer-wise message passing while dynamically filtering auxiliary edges and purifying node features based on target behavior representations, preventing noise accumulation across propagation layers, and (2) \textit{target-anchored contrastive alignment} to further regularize auxiliary embeddings by aligning them with target preference space through self-supervised learning, ensuring consistency between auxiliary and target representations.
\subsubsection{\textbf{Base Encoding.}}
Similar to Section~\ref{sec:unobserved_base}, we first compute base user/item representations that serve as the starting point for subsequent environment-specific modeling. Specifically, we obtain global and target representations using LightGCN encoder as follows:
\begin{equation}
\mathbf{E}^{\mathrm{glo}}=\mathrm{LGCN}(\mathbf{E}^{\mathrm{init}},\mathcal{G}_{\mathrm{glo}}),
\qquad
\mathbf{E}^{\mathrm{tar}}=\mathrm{LGCN}(\mathbf{E}^{\mathrm{glo}},\mathcal{G}_{\mathrm{tar}}),
\end{equation}

\vspace{0.25em}
\subsubsection{\textbf{Target-Gated Pruning Graph Encoder}}
Given an auxiliary behavior graph $\mathcal{G}_{b}$, we encode it with a layer-wise target-gated pruning operator.
For each layer $l$, we denote the auxiliary embeddings as $\mathbf{e}^{b,(l)}_{u}$ and $\mathbf{e}^{b,(l)}_{i}$, initialized by $\mathbf{e}^{b,(0)}=\mathbf{e}^{\mathrm{glo}}$.
To prevent auxiliary noise from contaminating the target encoder while allowing auxiliary representations to align with the target preference space, we use the target embeddings $\mathbf{e}^{\mathrm{tar}}_{u}$ and $\mathbf{e}^{\mathrm{tar}}_{i}$ as fixed anchors by stopping their gradient flow.
Throughout this section, we denote $\mathbf{t}_{x}=\mathrm{detach}(\mathbf{e}^{\mathrm{tar}}_{x})$ for any node $x$.

\noindent\textbf{Target-gated purification.}
We construct a feature-wise gate $\boldsymbol{\alpha}^{b,(l)}\in(0,1)^d$ that determines how much each feature dimension should rely on auxiliary signals versus target anchors.
The gate and purified representation are computed as:
\begin{equation}
\boldsymbol{\alpha}^{b,(l)}_{x}
= \sigma\!\big(\mathbf{W}^{b,(l)}_{x}\mathbf{e}^{b,(l)}_{x}+\mathbf{W}^{b,(l)}_{t}\mathbf{t}_{x}+\mathbf{b}^{b,(l)}\big),
\end{equation}
\begin{equation}
\mathbf{g}^{b,(l)}_{x}
= \boldsymbol{\alpha}^{b,(l)}_{x}\odot \mathbf{e}^{b,(l)}_{x}
+ \big(\mathbf{1}-\boldsymbol{\alpha}^{b,(l)}_{x}\big)\odot \mathbf{t}_{x},
\end{equation}
where $x\in\mathcal{U}\cup\mathcal{I}$.
This adaptive interpolation selectively filters auxiliary features inconsistent with the target preference space, mitigating noise accumulation across layers.

\vspace{0.25em}
\noindent\textbf{Learnable edge pruning.}
Beyond feature-level refinement, we perform structure-level pruning to remove unreliable auxiliary edges.
For each edge $(u,i)\in\mathcal{E}_{b}$, we predict a binary keep/drop decision using the purified representations:
\begin{equation}
\boldsymbol{\ell}^{b,(l)}_{ui}
= \mathbf{W}^{b,(l)}_{2}\big[\mathbf{g}^{b,(l)}_{u}\ \Vert\ \mathbf{g}^{b,(l)}_{i}\big]+\mathbf{b}^{b,(l)}_{2}\in\mathbb{R}^{2},
\end{equation}
\begin{equation}
\mathbf{y}^{b,(l)}_{ui}=\mathrm{GumbelSoftmax}(\boldsymbol{\ell}^{b,(l)}_{ui};\tau),\quad
z^{b,(l)}_{ui}=\mathbf{y}^{b,(l)}_{ui}[0]\in\{0,1\}.
\end{equation}
Where, $z^{b,(l)}_{ui}=1$ indicates the edge is kept, and $z^{b,(l)}_{ui}=0$ means it is pruned.

\vspace{0.25em}
\noindent\textbf{Similarity-based reweighting and normalization.}
For surviving edges, we assign confidence weights reflecting both angular alignment and magnitude consistency.
Following the approach in Section~4.1.3, we compute the fused similarity as:
\begin{equation}
w^{b,(l)}_{ui}
=
\frac{1}{2}\Big(1+\cos(\mathbf{g}^{b,(l)}_{u},\mathbf{g}^{b,(l)}_{i})\Big)\,
\exp\!\left(-\frac{\|\mathbf{g}^{b,(l)}_{u}-\mathbf{g}^{b,(l)}_{i}\|_{2}^{2}}{2\sigma^{2}}\right).
\end{equation}
The final edge weight combines the pruning decision with this similarity score:
$\bar{w}^{b,(l)}_{ui}=z^{b,(l)}_{ui}\cdot w^{b,(l)}_{ui}$.
To prevent high-degree nodes from dominating information aggregation while ensuring low-degree nodes receive sufficient signals, we apply symmetric normalization based on the pruned structure:
\begin{equation}
d^{b,(l)}_{u}=\sum_{i\in \mathcal{N}_{b}(u)} z^{b,(l)}_{ui},\quad
d^{b,(l)}_{i}=\sum_{u\in \mathcal{N}_{b}(i)} z^{b,(l)}_{ui},
\end{equation}
\begin{equation}
\tilde{w}^{b,(l)}_{ui}=\frac{\bar{w}^{b,(l)}_{ui}}{\sqrt{d^{b,(l)}_{u}\cdot d^{b,(l)}_{i}}}.
\end{equation}
This normalization mitigates the risk that high-degree nodes mix excessive information and dominate representations, while preventing low-degree nodes from being under-represented.

\vspace{0.25em}
\noindent\textbf{Message passing.}
The item representation is updated by aggregating messages from its pruned neighborhood:
\begin{equation}
\mathbf{e}^{b,(l+1)}_{i}=\sum_{u\in \mathcal{N}_{b}(i)} \tilde{w}^{b,(l)}_{ui}\,\mathbf{e}^{b,(l)}_{u},
\end{equation}
and user updates are defined symmetrically.
After $L$ layers, we obtain the refined auxiliary embedding $\mathbf{E}^{b}$ for each auxiliary behavior $b$.

\subsubsection{\textbf{Target-Anchored Contrastive Alignment}}
Although the pruning encoder suppresses noisy auxiliary relations, the resulting embeddings may still deviate from the target preference space, especially early in training.
To further regularize auxiliary representations, we align each auxiliary view with the target embedding using contrastive learning, treating the detached target embedding $\mathbf{t}_{x}$ as a stable anchor.
We stop gradient flow to the target encoder to prevent auxiliary noise from contaminating the target space and to avoid instability from early-stage target embeddings.

The user-side alignment loss for behavior $b$ is:
\begin{equation}
\mathcal{L}^{user,b}_{ssl}
= - \sum_{u\in\mathcal{U}}
\log
\frac{\exp\big(\mathrm{sim}(\mathbf{t}_{u},\mathbf{e}^{b}_{u})/\tau\big)}
{\sum_{u'\in\mathcal{U}} \exp\big(\mathrm{sim}(\mathbf{t}_{u},\mathbf{e}^{b}_{u'})/\tau\big)}.
\end{equation}
We compute the item-side loss $\mathcal{L}^{item,b}_{ssl}$ analogously, and aggregate across all auxiliary behaviors:
\begin{equation}
\mathcal{L}^{(ob)}_{ssl}=\sum_{b\in\mathcal{B}\setminus\{b_\mathrm{tar}\}} \big(\mathcal{L}^{user,b}_{ssl}+\mathcal{L}^{item,b}_{ssl}\big).
\end{equation}

\subsection{Training \& Inference}

\subsubsection{Training}

We train BOAR end-to-end with environment-specific objectives that address their distinct challenges.
For training, we construct a triplet set $\mathcal{D}$ , where each triplet $(u,i,j)$ consists of a user $u$, a positive item $i$ with $(u,i) \in \mathcal{E}_{\mathrm{tar}}$, and a negative item $j$ with $(u,j) \notin \mathcal{E}_{\mathrm{tar}}$ .

\vspace{0.25em}
\noindent\textbf{Auxiliary-Unobserved Environment.}
In this environment, the primary challenge is recovering hidden preferences from incomplete and biased observations.
We compute the preference score using the target embeddings:
\begin{equation}
s_{ui}^{(unob)} = {\mathbf{e}}^{\mathrm{tar}}_{u}{}^{\top}{\mathbf{e}}^{\mathrm{tar}}_{i},
\end{equation}
where ${\mathbf{e}}^{buy}$ denotes the target embeddings from Section~\ref{sec:hidden_miner}.
To address observation bias inherent in the mined candidate edges, we adopt SNIPS (Self-Normalized Inverse Propensity Score) reweighting for the ranking loss.
For each positive interaction $(u,i)\in\mathcal{E}_\mathrm{tar}$, we compute the debiasing weight $\omega_i$  (detailed derivation in Appendix).
The SNIPS-weighted BPR loss downweights over-represented popular items:
\begin{equation}
\mathcal{L}^{(unob)}_{rank}(\theta_0)
= - \sum_{(u,i,j)\in\mathcal{D}} \omega_i \cdot \log\sigma(s_{ui}^{(unob)} - s_{uj}^{(unob)}),
\end{equation}
where $\theta_0$ denotes all parameters in the auxiliary-unobserved environment.
The complete objective combines debiasing, robust transfer, and ranking:
\begin{equation}
\mathcal{L}^{(unob)}(\theta_0)
= \mathcal{L}^{(unob)}_{rank}(\theta_0)
+ \lambda_1 \mathcal{L}_{dom}
+ \lambda_2 \mathcal{L}^{(unob)}_{ssl}.
\end{equation}

\vspace{0.25em}
\noindent\textbf{Auxiliary-Observed Environment.}
After obtaining purified embeddings for each auxiliary behavior via target-gated pruning graph encoder, we aggregate them to produce the final representation.
Following prior works~\cite{}, we employ target attention (TA) to adaptively weight behavior embeddings based on their relevance to the target behavior:
\begin{equation}
\mathbf{E}^{\text{agg}} = \text{TA}\left(\mathbf{E}^{\mathrm{tar}}, \{\mathbf{E}^{b}\}_{b \in \mathcal{B}}\right),
\end{equation}
where $\text{TA}(k, q)$ denotes applying target attention to aggregate keys $k$ with query $q$, and $\mathcal{B}$ denotes the set of all behaviors including the target.

We compute the preference score as the inner product of aggregated user and item embeddings:
\begin{equation}
s_{ui}^{(ob)} = \mathbf{e}_{u}^{\text{agg}\top}\mathbf{e}_{i}^{\text{agg}}.
\end{equation}
The ranking loss is computed using standard BPR:
\begin{equation}
\mathcal{L}^{(ob)}_{rank}(\theta_1)
= - \sum_{(u,i,j) \in \mathcal{D}} \log\sigma(s_{ui}^{(ob)} - s_{uj}^{(ob)}),
\end{equation}
where $\theta_1$ denotes all parameters in the auxiliary-observed environment.
The complete objective combines ranking and contrastive alignment:
\begin{equation}
\mathcal{L}^{(ob)}(\theta_1)
= \mathcal{L}^{(ob)}_{rank}(\theta_1)
+ \lambda_3 \mathcal{L}^{(ob)}_{ssl}.
\end{equation}

\subsubsection{Inference}

At inference, we route each user-item pair to its environment-specific scorer based on auxiliary observability.
For a pair $(u,i)$, the final prediction score is computed via hard environment gating:
\begin{equation}
\hat{r}_{ui}
=
E_{ui}\cdot s_{ui}^{(ob)}
+
(1-E_{ui})\cdot s_{ui}^{(unob)},
\end{equation}
where $E_{ui}$ is the environment indicator (Eq.~\ref{eq:env_indicator}).
This hard gating ensures that pairs with auxiliary interactions are scored by the noise-suppressed multi-behavior model, while pairs without auxiliary evidence are scored by the debiased hidden preference model, preventing negative transfer between heterogeneous environments.

==> sections/999Algorithms.tex <==
%%%%%%%%%%%%%%%%%
\vspace{-10pt}
\begin{algorithm}[h]
\small{
\caption{Debiased Densification Module ($f_0$)}
\label{alg:f0}
\DontPrintSemicolon
\setlength{\textfloatsep}{0cm}
\setlength{\floatsep}{0cm}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{
Global embeddings $\mathbf{E}^{\mathrm{glo}}$, 
Target embeddings $\mathbf{E}^{\mathrm{tar}}$,\\
IPS weights for debiasing $\{\omega_i\}_{i\in\mathcal{I}}$
}

\Output{
Updated densification module $f_0$
}

\BlankLine
\tcc{Auxiliary-Invariant Learning (Sec.~4.2.1)}
Construct $\mathcal{S}_{\mathrm{adv}}$ and compute adversarial loss $\mathcal{L}_{adv}$ (Eq.~(6)) \;

\BlankLine
\tcc{Target Hidden Preference Mining (Sec. 4.2.2)}
Retrieve candidate pairs using angular LSH \;
Select target-aligned pairs via learnable edge selection (Eq.~(7))\;
Construct weighted densified target graph $\tilde{\mathbf{A}}_{\mathrm{tar}}$ (Eq.~(9)) \;

\BlankLine
\tcc{Debiased Densification Learning (Sec. 4.2.3)}
Generate densified embeddings $\tilde{\mathbf{E}}_{\mathrm{tar}} = \mathrm{LGCN}(\tilde{\mathbf{A}}_{\mathrm{tar}}, \mathbf{E}^{\mathrm{glo}})$\;
Compute contrastive loss $\mathcal{L}_{dense}$ (Eq.~(10)) \;
Compute ranking loss with SNIPS weighting $\mathcal{L}_{rank}$ (Eq.~(11)) \;

\BlankLine
% \tcc{Overall Objective}
Minimize 
$\mathcal{L}_{rank} + \lambda_{adv}\mathcal{L}_{adv} + \lambda_{dense}\mathcal{L}_{dense}$ (Eq.~(12)) \;
}
\end{algorithm}
\vspace{-10pt}
%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\small{
\caption{Target-Guided Refinement Module ($f_1$)}
\label{alg:f1}
\DontPrintSemicolon
\setlength{\textfloatsep}{0cm}
\setlength{\floatsep}{0cm}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{
Global embeddings $\mathbf{E}^{\mathrm{glo}}$, 
Target embeddings $\mathbf{E}^{\mathrm{tar}}$
}
\Output{
Updated refinement module $f_1$
}

\BlankLine
\tcc{Target-Guided Aux. Graph Refinement (Sec.~4.3.1)}
For each auxiliary behavior graph $\mathcal{G}_b$: \;
\Indp For each LGCN layer $l$: \;
    \Indp 
    Refine features using target-guided gating (Eq.~(13)) \;
    Prune target-misaligned edges (Eq.~(14)) \;
\Indm Construct layer-wise refined graphs 
$\tilde{\mathbf{A}}_b = \{\tilde{\mathbf{A}}^{b,(l)}\}_{l=1}^{L}$ (Eq.~(15)) \;
Generate refined embeddings $\tilde{\mathbf{E}}_{b} = \mathrm{LGCN}(\tilde{\mathbf{A}}_{b}, \mathbf{E}^{\mathrm{glo}})$ \;
\Indm

\BlankLine
\tcc{Target-Guided Preference Learning (Sec.~4.3.2)}
Compute contrastive loss $\mathcal{L}_{refine}$ (Eq.~(16)) \;
Compute final embeddings and ranking loss $\mathcal{L}_{rank}$ (Eq.~(17)) \;

\BlankLine
% \tcc{Overall Objective}
Minimize  $\mathcal{L}_{rank} + \lambda_{refine}\mathcal{L}_{refine}$ (Eq.~(18)) \;
}
\end{algorithm}
\vspace{-10pt}
%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\small{
\caption{Unified Modular Learning and Inference}
\label{alg:unified}
\DontPrintSemicolon
\setlength{\textfloatsep}{0cm}
\setlength{\floatsep}{0cm}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{
Target interaction set $\mathcal{E}_{\mathrm{tar}}$, 
auxiliary interaction set $\mathcal{E}_{\mathrm{aux}}$,\\
environment-specific modules $\{f_0, f_1\}$
}
\Output{
Updated model parameters; target behavior predictions
}

Compute global and target embeddings for each module

\BlankLine
\tcc{Training Phase}
For each $(u,i)\in\mathcal{E}_{\mathrm{tar}}$: \;
\Indp
Compute environment indicator 
$\hat e = \mathbb{I}[(u,i)\in\mathcal{E}_{\mathrm{aux}}]$ \;
Update module $f_{\hat e}$ using loss $\mathcal{L}_{f_{\hat e}}(u,i)$ \;
\Indm

\BlankLine
\tcc{Inference Phase}
For each $(u,i)$ to be ranked: \;
\Indp
Compute environment indicator 
$\hat e = \mathbb{I}[(u,i)\in\mathcal{E}_{\mathrm{aux}}]$ \;
Predict ranking score using module $f_{\hat e}$ \;
\Indm
}
\end{algorithm}
\vspace{-10pt}


==> table/abl_assignment.tex <==
\begin{table}
\caption{Ablation study on modular assignment strategy 
         in the general setting.}
\label{tab:abl_assign}
\begin{tabular}{l|cc|cc|cc}
\toprule
Variant & \multicolumn{2}{c|}{Tmall} & 
          \multicolumn{2}{c|}{Taobao} & 
          \multicolumn{2}{c}{JData} \\
        & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 \\
\midrule
BOAR (soft)    & & & & & & \\
Hard ($E_{ui}$) & & & & & & \\
Average (0.5)  & & & & & & \\
\bottomrule
\end{tabular}
\end{table}

==> table/abl_unob.tex <==
\begin{table}[t]
  \centering
  \caption{Ablation study on debiased densification module.}
  \label{tab:abl_unob}

  \begingroup
  \setlength{\tabcolsep}{2.5pt}
  \renewcommand{\arraystretch}{1.1}
  % \small
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l cc cc cc}
    \toprule
    \multirow{2}{*}{Model variant}
    & \multicolumn{2}{c}{Tmall}
    & \multicolumn{2}{c}{Taobao}
    & \multicolumn{2}{c}{JData} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
    & HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 \\
    \midrule

    \textbf{\proposed}
    & \textbf{0.1245} & \textbf{0.0768}
    &  \textbf{0.0310} & \textbf{0.0175}
    & \textbf{0.5509} & \textbf{0.3743} \\
    \midrule

    w/o $\mathcal{L}_{\mathrm{dense}}$
    & 0.0833 & 0.0469
    & 0.0234 & 0.0146
    & 0.4060 & 0.2583 \\

    w/o $\mathcal{L}_{\mathrm{adv}}$
    & 0.1126 & 0.0675
    & 0.0285 & 0.0163
    & 0.5331 & 0.3580 \\

    w/o SNIPS
    &  0.1184 &  0.0693
    & 0.0302 &  0.0169
    &  0.5353 &  0.3700 \\

    % w/o Hard approx.
    % & 0.1048 & 0.0572
    % & \textbf{0.0316} & 0.0171
    % & 0.4890 & 0.3073 \\
    \bottomrule
  \end{tabular}}
  \endgroup
  \vspace{-0.3cm}
\end{table}


==> table/inference_time.tex <==
\begin{table}[h]
  \centering
  \caption{Efficiency analysis: comparison of training time (sec), inference time (sec), and model size (in millions). Training time denotes the average time per epoch, and inference time denotes the time to generate recommendations for all users. }
  \begingroup
  \renewcommand{\arraystretch}{1.}
  % \setlength{\tabcolsep}{5pt}
  % \small
  \resizebox{0.95\linewidth}{!}{
  \begin{tabular}{llcccc}
    \toprule
    \textbf{Dataset} & \textbf{Metric} & \textbf{MuLe} & \textbf{HGIB} & \textbf{MEMBER} & \textbf{BOAR} \\
    \midrule
      & Train time  & 81.47s & 86.46s & 164.85s & 107.36s \\
     \textbf{Tmall} & Inference time   & 12.52s & 11.24s & 12.82s & 8.80s \\
      & \#Parameters  & 3.44M    & 3.44M    & 3.44M    & 3.45M            \\
    \midrule
      & Train time  & 70.22s & 64.43s & 116.97s & 86.45s \\
     \textbf{Taobao} & Inference time & 21.69s & 19.66s & 22.84s & 15.90s \\
      & \#Parameters  & 5.65M    & 5.66M    & 5.65M    & 5.66M             \\
    \midrule
      & Train time   & 100.12s & 90.83s & 178.49s & 148.98s \\
     \textbf{JData} & Inference time & 5.92s  & 5.69s  & 6.22s  & 4.77s \\
      & \#Parameters  & 7.55M    & 7.56M    & 7.55M    & 7.56M            \\
    \bottomrule
  \end{tabular}}
  \endgroup
  \label{tab:inference_time}
\end{table}


==> table/ob_performance.tex <==
\begin{table*}[b]
  \centering
  \caption{Auxiliary-observed performance across three datasets.
  Best and second-best results are highlighted in \textbf{bold} and \underline{underlined}, respectively.}
  \label{tab:aux_observed}

  % ---- local formatting (kept inside this table only) ----
  \begingroup
  \setlength{\tabcolsep}{2.5pt} % column padding (tune: 1.5~4pt)
  \renewcommand{\arraystretch}{1}
  \newcommand{\best}[1]{\textbf{#1}}
  \newcommand{\second}[1]{\underline{#1}}  
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllccccccccccccc}
      \toprule
      \multirow{2}{*}{\textbf{Dataset}} &
      \multirow{2}{*}{\textbf{Types}} &
      \multirow{2}{*}{\textbf{Metric}} &
      \multicolumn{2}{c}{\textbf{Single-Behavior}} &
      \multicolumn{11}{c}{\textbf{Multi-Behavior}} \\
      \cmidrule(lr){4-5} \cmidrule(lr){6-15}
      & & & \textbf{MF-BPR} & \textbf{LGCN} &
      \textbf{LGCN-G} & \textbf{MB-GMN} & \textbf{CIGF} & \textbf{CRCGN} &
      \textbf{BCIPM} & \textbf{MB-HGCN} & \textbf{COPF}$\,\,$ & \textbf{MuLe}$\,\,$ &
      \textbf{HGIB} & \textbf{MEMBER} & \textbf{BOAR} \\
      \midrule

      \multirow{4}{*}{\textbf{Tmall}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.0427 & 0.0391 & 0.1339 & 0.0452 & 0.0662 & 0.1067 & 0.1407 & 0.1462 & 0.1670 & 0.2088 & 0.2415 & \underline{0.3507} & \textbf{0.3674} \\
      & & \textbf{NDCG@10} & 0.0210 & 0.0201 & 0.0681 & 0.0228 & 0.0333 & 0.0569 & 0.0765 & 0.0778 & 0.0810 & 0.1158 & 0.1274 & \underline{0.1730} & \textbf{0.1787} \\ \cmidrule(lr){2-16}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.3996 & 0.3773 & 0.4256 & 0.3740 & 0.4062 & 0.4167 & 0.3997 & 0.3962 & 0.4070 & \second{0.4577} & 0.4527 & 0.4554 & \best{0.4588} \\
      & & \textbf{NDCG@10} & 0.1891 & 0.1765 & 0.2044 & 0.1834 & 0.1933 & 0.1969 & 0.1905 & 0.1878 & 0.1921 & 0.2224 & 0.2202 & \second{0.2226} & \best{0.2232} \\
      \midrule

      \multirow{4}{*}{\textbf{Taobao}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.0239 & 0.0178 & 0.1049 & 0.0498 & 0.0649 & 0.1007 & 0.1270 & 0.1639 & 0.1543 & 0.2121 & 0.2582 & \underline{0.3183} & \textbf{0.3443} \\
      & & \textbf{NDCG@10} & 0.0130 & 0.0095 & 0.0591 & 0.0198 & 0.0327 & 0.0564 & 0.0711 & 0.0950 & 0.0895 & 0.1346 & 0.1620 & \underline{0.1640} & \textbf{0.1886} \\ \cmidrule(lr){2-16}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.4587 & 0.4619 & 0.4938 & 0.4736 & 0.4849 & 0.5007 & 0.5070 & 0.5239 & 0.5343 & 0.5690 & \best{0.5797} & 0.5279 & \second{0.5694} \\
      & & \textbf{NDCG@10} & 0.2252 & 0.2290 & 0.2458 & 0.2318 & 0.2327 & 0.2464 & 0.2511 & 0.2650 & 0.2695 & 0.3050 & \best{0.3238} & 0.2738 & \second{0.3057} \\
      \midrule

      \multirow{4}{*}{\textbf{Jdata}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.3674 & 0.2779 & 0.4163 & 0.2815 & 0.3650 & 0.4730 & 0.5252 & 0.5234 & 0.4497 & 0.5837 & 0.6502 & \underline{0.6589} & \textbf{0.6960} \\
      & & \textbf{NDCG@10} & 0.2234 & 0.1704 & 0.2411 & 0.1652 & 0.2272 & 0.2980 & 0.3158 & 0.3402 & 0.2723 & 0.4209 & \underline{0.4667} & 0.4332 & \textbf{0.4795} \\ \cmidrule(lr){2-16}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.7324 & 0.7189 & 0.7100 & 0.6935 & 0.7150 & 0.7230 & 0.7252 & 0.7234 & 0.7197 & 0.7693 & \best{0.7826} & 0.7383 & \second{0.7730} \\
      & & \textbf{NDCG@10} & 0.3751 & 0.4461 & 0.4372 & 0.4392 & 0.4427 & 0.4380 & 0.4458 & 0.4402 & 0.4423 & 0.4749 & \best{0.5340} & 0.4920 & \second{0.5160} \\
      \bottomrule
    \end{tabular}%
  }\vspace{-0.4cm}
  \endgroup
\end{table*}


==> table/overall_ori.tex <==
\begin{table*}[t]
  \centering
  \caption{Performance comparison on three datasets. 
  $^*$ indicates statistical significance for $p<0.001$ under t-test compared to the best baseline.}
  \label{tab:overall_performance}

  % ---- local formatting (kept inside this table only) ----
  \begingroup
  \setlength{\tabcolsep}{2.5pt} % column padding (tune: 1.5~4pt)
  \renewcommand{\arraystretch}{1}
  % \scriptsize % or \footnotesize
    
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{lllcccccccccccccc}
      \toprule
      \multirow{2}{*}{\textbf{Dataset}} &
      \multirow{2}{*}{\textbf{Types}} &
      \multirow{2}{*}{\textbf{Metric}} &
      \multicolumn{2}{c}{\textbf{Single-Behavior}} &
      \multicolumn{12}{c}{\textbf{Multi-Behavior}} \\
      \cmidrule(lr){4-5} \cmidrule(lr){6-17}
      & & & \textbf{MF-BPR} & \textbf{LGCN} &
      \textbf{LGCN-G} & \textbf{MB-GMN} & \textbf{CIGF} & \textbf{CRCGN} &
      \textbf{BCIPM} & \textbf{MB-HGCN} & \textbf{COPF}$\,\,$ & \textbf{MuLe}$\,\,$ &
      \textbf{HGIB} & \textbf{MEMBER} & \textbf{BOAR}$_{\text{\textbf{base}}}$ & \textbf{BOAR} \\
      \midrule

      \multirow{6}{*}{\textbf{Tmall}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.0427 & 0.0391 & 0.1339 & 0.0452 & 0.0662 & 0.1067 & 0.1407 & 0.1462 & 0.1670 & 0.2088 & 0.2415 & \underline{0.3507} & - & \textbf{0.3739$^*$} \\
      & & \textbf{NDCG@10} & 0.0210 & 0.0201 & 0.0681 & 0.0228 & 0.0333 & 0.0569 & 0.0765 & 0.0778 & 0.0810 & 0.1158 & 0.1274 & \underline{0.1730} & - & \textbf{0.1821$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Unobserved}} &
      \textbf{HR@10}   & 0.0662 & 0.0692 & 0.0835 & 0.0298 & 0.0492 & 0.0396 & 0.0402 & 0.0329 & 0.0355 & 0.0549 & 0.0420 & \underline{0.0948} & - & \textbf{0.1390$^*$} \\
      & & \textbf{NDCG@10} & 0.0335 & 0.0382 & 0.0425 & 0.0154 & 0.0237 & 0.0192 & 0.0196 & 0.0146 & 0.0168 & 0.0289 & 0.0213 & \underline{0.0594} & - & \textbf{0.0828$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.3996 & 0.3773 & 0.4256 & 0.3740 & 0.4062 & 0.4167 & 0.3997 & 0.3962 & 0.4070 & \underline{0.4577} & 0.4527 & 0.4554 & - & \textbf{0.4587$^*$} \\
      & & \textbf{NDCG@10} & 0.1891 & 0.1765 & 0.2044 & 0.1834 & 0.1933 & 0.1969 & 0.1905 & 0.1878 & 0.1921 & 0.2224 & 0.2202 & \underline{0.2226} & - & \textbf{0.2232$^*$} \\
      \midrule

      \multirow{6}{*}{\textbf{Taobao}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.0239 & 0.0178 & 0.1049 & 0.0498 & 0.0649 & 0.1007 & 0.1270 & 0.1639 & 0.1543 & 0.2121 & 0.2582 & \underline{0.3183} & - & \textbf{0.3450$^*$} \\
      & & \textbf{NDCG@10} & 0.0130 & 0.0095 & 0.0591 & 0.0198 & 0.0327 & 0.0564 & 0.0711 & 0.0950 & 0.0895 & 0.1346 & 0.1620 & \underline{0.1640} & - & \textbf{0.1886$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Unobserved}} &
      \textbf{HR@10}   & 0.0167 & 0.0124 & 0.0212 & 0.0182 & 0.0206 & 0.0152 & 0.0148 & 0.0153 & 0.0182 & 0.0248 & \underline{0.0252} & 0.0221 & - & \textbf{0.0370$^*$} \\
      & & \textbf{NDCG@10} & 0.0093 & 0.0068 & 0.0105 & 0.0094 & 0.0102 & 0.0089 & 0.0085 & 0.0088 & 0.0075 & 0.0137 & \underline{0.0147} & 0.0118 & - & \textbf{0.0202$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.4587 & 0.4619 & 0.4938 & 0.4736 & 0.4849 & 0.5007 & 0.5070 & 0.5239 & 0.5343 & 0.5690 & \textbf{0.5797} & 0.5279 & - & \underline{0.5700} \\
      & & \textbf{NDCG@10} & 0.2252 & 0.2290 & 0.2458 & 0.2318 & 0.2327 & 0.2464 & 0.2511 & 0.2650 & 0.2695 & 0.3050 & \textbf{0.3238} & 0.2738 & - & \underline{0.3079} \\
      \midrule

      \multirow{6}{*}{\textbf{Jdata}} & \multirow{2}{*}{\textbf{General}} &
      \textbf{HR@10}   & 0.3674 & 0.2779 & 0.4163 & 0.2815 & 0.3650 & 0.4730 & 0.5252 & 0.5234 & 0.4497 & 0.5837 & 0.6502 & \underline{0.6589} & - & \textbf{0.6971$^*$} \\
      & & \textbf{NDCG@10} & 0.2234 & 0.1704 & 0.2411 & 0.1652 & 0.2272 & 0.2980 & 0.3158 & 0.3402 & 0.2723 & 0.4209 & \underline{0.4667} & 0.4332 & - & \textbf{0.4937$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Unobserved}} &
      \textbf{HR@10}   & 0.3610 & 0.2679 & 0.3671 & 0.2295 & 0.2971 & 0.3241 & 0.3273 & 0.4164 & 0.2610 & \underline{0.4749} & 0.4566 & 0.3947 & - & \textbf{0.5438$^*$} \\
      & & \textbf{NDCG@10} & 0.2002 & 0.1432 & 0.2103 & 0.1415 & 0.1854 & 0.1886 & 0.1836 & 0.2588 & 0.1743 & \underline{0.2975} & 0.2769 & 0.2403 & - & \textbf{0.3665$^*$} \\ \cmidrule(lr){2-17}
      & \multirow{2}{*}{\textbf{Observed}} &
      \textbf{HR@10}   & 0.7324 & 0.7189 & 0.7100 & 0.6935 & 0.7150 & 0.7230 & 0.7252 & 0.7234 & 0.7197 & 0.7693 & \textbf{0.7826} & 0.7383 & - & \underline{0.7757} \\
      & & \textbf{NDCG@10} & 0.3751 & 0.4461 & 0.4372 & 0.4392 & 0.4427 & 0.4380 & 0.4458 & 0.4402 & 0.4423 & 0.4749 & \textbf{0.5340} & 0.4920 & - & \underline{0.5273} \\
      \bottomrule
    \end{tabular}%
  }\vspace{-0.4cm}
  \endgroup
\end{table*}

==> table/soft_gating.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on gating strategy (dummy).}
\label{tab:gating_3split_1col}
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.05}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{Model Variant}
& \multicolumn{6}{c|}{Tmall}
& \multicolumn{6}{c|}{Taobao}
& \multicolumn{6}{c}{JData} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}\cmidrule(lr){14-19}
& \multicolumn{2}{c|}{General} & \multicolumn{2}{c|}{Observed} & \multicolumn{2}{c|}{Unobserved}
& \multicolumn{2}{c|}{General} & \multicolumn{2}{c|}{Observed} & \multicolumn{2}{c|}{Unobserved}
& \multicolumn{2}{c|}{General} & \multicolumn{2}{c|}{Observed} & \multicolumn{2}{c}{Unobserved} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\cmidrule(lr){14-15}\cmidrule(lr){16-17}\cmidrule(lr){18-19}
& HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10
& HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10
& HR@10 & NDCG@10 & HR@10 & NDCG@10 & HR@10 & NDCG@10 \\
\midrule
Hard gating
& \textbf{0.3674} & \textbf{0.1787} & \textbf{0.3920} & \textbf{0.1965} & \textbf{0.1245} & \textbf{0.0768}
& \textbf{0.3443} & \textbf{0.1886} & \textbf{0.3580} & \textbf{0.1995} & \textbf{0.0310} & \textbf{0.0175}
& \textbf{0.6960} & \textbf{0.4795} & \textbf{0.7210} & \textbf{0.5010} & \textbf{0.5509} & \textbf{0.3743} \\
Soft gating
& 0.1715 & 0.0836 & 0.1850 & 0.0910 & 0.0600 & 0.0350
& 0.1110 & 0.0615 & 0.1200 & 0.0660 & 0.0200 & 0.0110
& 0.5286 & 0.3575 & 0.5400 & 0.3660 & 0.4000 & 0.2550 \\
\bottomrule
\end{tabular}%
}
\end{table}

